A workload-adaptive mechanism for linear queries under local differential privacy

We propose a new mechanism to accurately answer a user-provided set of linear counting queries under local differential privacy (LDP). Given a set of linear counting queries (the workload) our mechanism automatically adapts to provide accuracy on the workload queries. We define a parametric class of mechanisms that produce unbiased estimates of the workload, and formulate a constrained optimization problem to select a mechanism from this class that minimizes expected total squared error. We solve this optimization problem numerically using projected gradient descent and provide an efficient implementation that scales to large workloads. We demonstrate the effectiveness of our optimization-based approach in a wide variety of settings, showing that it outperforms many competitors, even outperforming existing mechanisms on the workloads for which they were intended.

==> 2 <==
\section{Related Works}

The problem we considered in this work, and the mechanism we proposed was inspired by a large body of related work in the central and local model of differential privacy.

Answering linear queries under central differential privacy is a widely studied topic \cite{barak2007privacy,li2015matrix,mckenna2018optimizing,bhaskara2012unconditional,li2012adaptive}.  Many state of the art mechanisms for this task, like the matrix mechanism \cite{li2010optimizing}, achieve privacy by adding Laplace or Gaussian noise to a carefully selected set of ``strategy queries''.  This query strategy is tailored to the workload, and can even be optimized for it, as the matrix mechanism does.  The optimization problem posed by the matrix mechanism has been studied extensively theoretically \cite{li2010optimizing,li2015lower}, and several algorithms have been proposed to solve it or approximately solve it \cite{yuan2012low,li2012adaptive,yuan2016convex,mckenna2018optimizing}.  While similar in spirit to our mechanism, the optimization problem underlying the matrix mechanism is different than ours, as they search over a different space of mechanisms not tailored to local differential privacy.   

While answering linear queries under local differential privacy has recieved considerably less attention, any mechanism designed for the central model of differential privacy can be easiliy adapted to the local model simply by executing it independently for each single-user database.  This approach has been studied theoretically with the Gaussian mechanism \cite{bassily2018linear} and the matrix mechanism \cite{edmonds2019power}.  The main problem with this approach is that it is not tailored to local differential privacy, so it does not work particularly well in practice. 
Another notable approach for this task casts it as a mean estimation problem, and uses LDP mechanisms designed for that \cite{blasiok2019towards}.  These works provide a thorough theoretical treatment of this problem.  For example, \ry{Raj: please provide some more details here}.  However, to our knowledge, the mechanism we propose offers the first practical treatment of the problem in it's full generality.  

More work has been done to answer specific, fixed workloads of general interest, such as histograms \cite{acharya2018,ye2018optimal,wang2017locally, warner1965randomized,erlingsson2014rappor}, range queries \cite{cormode2019answering}, and marginals \cite{cormode2018marginal}

%\ry{What about the Kairouz paper on Extremal mechanisms.  That is extremely relevant.  How does it fit in?}

%\paragraph*{Workload Answering  in Central Model} Answering linear queries under central differential privacy is a widely studied topic \cite{barak2007privacy,li2015matrix,mckenna2018optimizing,bhaskara2012unconditional,li2012adaptive}.  In this setup, the privacy is generally achieved by adding noise to the query answer. The amount of noise is  determined by the quantity called  \emph{sensitivity} of the query. To achieve $\epsilon$- privacy the random noise is added according to the Laplace distribution and for approximate $(\epsilon,\delta)$ -privacy Gaussian distribution  is used. In the work \cite{li2015matrix}, the \emph{matrix mechanism} is explained where the queries are answered based on query strategy that supports the workload so as to reduce the error. In \emph{HDMM}(High Dimensinal Matrix Mechanism) \cite{mckenna2018optimizing} an optimization  based algorithms are developed to handle large scale workload query. Comaperd to the matrix mechanism, the problem here has its own sets of challenges as mechanism has structural constraint and that adds complexity to solution of the optimization problems.  In \cite{yuan2012low}, workload decomposition technique is developed in order to minimize error. Our algorithm  is also workload decomposition based but in our case one of the factor of decomposition is strategy matrix $(\Q)$ which has probability constraint in each column and privacy constraint in  each row.

\paragraph*{Private Histogram Workload}
In \cite{acharya2018,ye2018optimal,wang2017locally,warner1965randomized,erlingsson2014rappor} mechanisms have been designed  for the purpose of private distribution estimation. In terms of workload, distribution estimation is answering to identity workload which is essentially estimation of Histogram. Also with the information of the Histogram  we can answer any linear workload by multiplying  the workload matrix with the privately estimated Histogram. Even though the private Histogram estimation can be thought of as a way of answering linear queries in general, they are not optimal in terms of error. In this work we develop mechanism that is adaptive to all general workload and all regime of privacy. A very concise description of the computational complexity, sample complexity and communication complexity etc for different range of privacy  can be found in \cite{acharya2018}.   

%\ry{I would not call it distribution estimation.  I would just use the terminology we have been using throughout the paper... i.e., Histogram workload or Histogram estimation}

%\ry{maybe add a discussion about how the optimal strategy for this workload is trivial in the central model, but not in the local model.   It's kind of interesting in my opinion}

%\ry{I would say more about the wang paper, they did a pretty in depth study on this problem}

 
\paragraph*{General Workload Answering} 
In the recent work \cite{bassily2018linear}, a private mechanism for general workload is proposed. The  privacy is achieved by adding Gaussian noise to the workload. The paper deals with answering both offline and online linear queries.  The analysis is carried out with the help of geometry of the differential privacy \cite{nikolov2013geometry}. Also in the paper  \cite{blasiok2019towards} the authors propose the algorithm based on two projection scheme named coarse projection method and chaining projection method. These methods are a refinement of the  projection method used in  \cite{bassily2018linear} and adopted from \cite{nikolov2013geometry}. The paper shows lower bound by \emph{separation number } of the space of the universe in the mean estimation problem.  In \cite{duchi2013local1,duchi2013local}, minimax rate of estimation under local privacy have been studied. In \cite{kairouz2014extremal}, the author posed the privacy-utility trade-off as a constrained maximization problem and show that optimal solution is contained in  a finite subset of \emph{extremal } mechanisms.

%\ry{there is a goldmine of theoretical results in these papers.  Would be nice to say more about those, and compare them to our own results}

%\ry{also need to mention the other factorization mechanism, and mention it's connections to the matrix mechanism}

\paragraph*{Specific Workload answering in LDP} In recent years, a few mechanisms are introduced specifically for answering some heavily used popular mechanism such as marginal workload and range query in the local model. \cite{cormode2018marginal} discusses hadamard matrix based  mechanism to answer k-way marginal queries. And in \cite{cormode2019answering} a hierarchical tree based mechanism is developed to answer all possible range query in the input domain.

%\ry{perhaps merge this with distribution estimation.  These are all instance of answering specific, fixed workloads.  In this case, Histogram, All Range, and k-way Marginals.}


==> extensions.tex <==
\section{Extensions}

In this section we describe a number of extensions to \mech that could improve it's scalability and/or utility even further.

\subsection{Non-negativity and Consistency}

Our basic mechanism has the appealing property of offering unbiased answers to the workload queries.  However, this can come at the cost of certain anomalies.  For example, the estimated answer to a workload query might be negative, even though the true answer could never be negative.  This motivates us to fix up this problem, reducing the variance at the cost of bias by imposing a non-negativity constraint on $\hat{\x}$.  The problem at hand is:

$$\hat{\x} = \argmin_{\x \geq 0} \norm{\W \x - \V \y}_2^2$$

The basic idea is to find the non-negative vector $\x$ such that $\W \x$ is as close as possible to the unbiased estimates $\V \y$.  A similar problem was considered by Li et al. and shown to offer utility improvements in the central model of differential privacy \cite{li2015matrix}.  Ideally, we would want to minimize over non-negative, \emph{integral} vectors $\x$, but imposing an integrality constraint poses some technical challenges so that constraint is relaxed.

\subsection{Workload-based domain reduction}

Workload-based domain reduction is a technique for losslessly compressing the workload.  It has been successfully applied in the centralized model of differential privacy \cite{li2015matrix,ektelo}.  The basic idea is that when two or more columns of $\W$ are identical, the duplicates can be removed without changing the problem.  Specifically, if column $u$ and $u'$ are the same, we can remove column $u'$ from $\W$ and pretend that all users of type $u'$ are actually of type $u$.  This reduces the size of the domain, and allows our techniques to scale better.  Furthermore, the optimization problem is typically easier to solve when the domain is smaller, so the utility may also improve from this preprocessing step.  It has been shown that applying workload-based domain reduction can never hurt the utility, and it can sometimes help a lot, depending on the workload.

\subsection{Parametric Optimization}

One thing we can do to extend the optimization framework is to consider searching over a parameterized strategy space, as done by \cite{mckenna2018optimizing} in the central model.  Specifically, we could define a class of strategies $\Q(\boldsymbol{\theta})$  parameterized by a vector $\boldsymbol{\theta}$.  Then we can optimize over $\boldsymbol{\theta}$ instead of $\Q$.  Since $\boldsymbol{\theta}$ might be considerably smaller than $\Q$, this could greatly improve the scalability of the optimization.  
Additionally, with the right parameterization, the parameterized strategy could have better utility than a general strategy due to the fact that the optimization problem is non-convex.
The parameterization must be carefully designed however, and should encode domain expertise about the workload and constraints.  

Some parameterizations might work well for one workload but not for others.  Existing LDP mechanisms can be thought of as an instance of parameterized strategies.  For example, Cormode et al. consider the class of hierarchical strategy matrices \cite{cormode2019answering}, parameterized by a branching factor $b$.  This parameterization was specifically designed to offer good utility on the workload of all range queries, and works pretty well for that but not for other workloads.

\subsection{High-Dimensional Workloads}

Many natural high-dimensional workloads can naturally be represented in matrix form in terms of \emph{Kronecker products}.  McKenna et al. showed that any workload consisting of queries from the expressive class of conjunctive counting queries can be represented as a union of Kronecker products \cite{mckenna2018optimizing}.  Thus, we might wonder whether it's possible to exploit this type of structure and efficiently solve the strategy optimization problem when using Algorithm \ref{alg:opt} directly becomes infeasible.

Kronecker products are a useful abstraction when each user holds more than one data item $u = (u^1, u^2, \dots) $.  For example, if $\Q_1$ is defined with respect to $u^1$ and $\Q_2$ is defined with respect to $u^2$ then $\Q_1 \otimes \Q_2$  is defined with respect to pairs $(u^1, u^2)$.  

We first show in Theorem \ref{thm:kronstrategy} that the Kronecker product of two LDP strategy matrices is still a LDP strategy matrix.

\begin{theorem}[Kronecker Strategy] \label{thm:kronstrategy}
Let $\Q_1$ be an $\epsilon_1$-LDP strategy matrix and $\Q_2$ be an $\epsilon_2$-LDP strategy matrix.  Then $ \Q = \Q_1 \otimes \Q_2 $ is an $(\epsilon_1 + \epsilon_2)$-LDP strategy matrix.  
\end{theorem}

\begin{proof}
todo
\end{proof}

A Kronecker product strategy is equivalent to a sequential composition of the mechanisms $\M(\cdot; \Q_1)$ and $\M(\cdot; \Q_2)$.  The following follows directly from the definition of Kronecker product

$$Pr[\M((u^1, u^2); \Q) = (o^1, o^2)] = Pr[\M(u^1; \Q_1) = o^1] \cdot Pr[\M(u^2; \Q_2) = o^2] $$

Remarkably, theorem \ref{thm:decomp} shows that the error of a Kronecker product strategy decomposes over the factors of the Kronecker product.  This is akin to what happens in the central model of differential privacy.  

\begin{theorem}[Error Decomposition] \label{thm:decomp}
Given a workload $ \W = \W_1 \otimes \W_2 $ and a strategy $\Q = \Q_1 \otimes \Q_2$, we have:

$$ L_{\W}(\Q) = L_{\W_1}(\Q_1) L_{\W_2}(\Q_2) $$
\end{theorem}


==> method.tex <==
\section{Approach}

\subsection{Error Derivations}

Let $\mathcal{Q}$ be the set of all valid strategy matrices (as per proposition \ref{prop1}).  Our goal is to find $\Q \in \mathcal{Q}$ such that the error of the corresponding LDP mechanism on the workload is minimized.  

We define error for a single workload query $\w$ to be:
$$ {\rm Error}(\w, \Q, \x) = \mathbb{E}[(\w^T \Q^{\dagger} \y - \w^T \x)^2] = {\rm Var}[\w^T \Q^{\dagger} \y]. $$
%The error on the workload $\W$ is then simply $ Error(\W, \Q, \x) = \sum_{\w \in \W} Error(\w, \Q, \x) $.  
Let $ \v = \w^T \Q^{\dagger} $ and $\q_u$ denote column $u$ of $\Q$, it is possible to show that the above variance can be expressed as follows:
\begin{align} \label{eq:variance}
& {\rm Var}[\w^T \Q^{\dagger} \y] =\nonumber \\ 
 &  \sum_{u \in \U} \x_u \big[ \w^T \Q^{\dagger} {\rm Diag}(\q_u) \Q^{{\dagger}T} \w - (\w^T \Q^{\dagger} \q_u)^2 \big]. 
\end{align}
Using Eq. \eqref{eq:variance}, we can efficiently calculate the expected error of the LDP mechanism on $\w$.  To calculate the error on the whole workload $\W$, we can simply compute $ \sum_{i} {\rm Var}[\w_i^T \Q^{\dagger} \y] $ using Eq. \eqref{eq:variance}.  This is the objective we would like to minimize.  

Note however that there is a dependence on the true data vector $\x$.  This is problematic because (1) we don't have access to $\x$ and (2) even if we did, computing $\Q$ based on it would violate differential privacy.  To overcome this, we use \emph{worst-case} error as our objective function.  The worst-case error occurs when all of the users have the same worst-case type.  Thus, our objective function becomes:
\begin{align} \label{eq:objective}
& L(\W, \Q) =\nonumber \\ &  \max_{u \in \U} \sum_{i} \big[ \w_i^T \Q^{\dagger} {\rm Diag}(\q_u) \Q^{{\dagger}T} \w_i - (\w_i^T \Q^{\dagger} \q_u)^2 \big].
\end{align}
\subsection{Optimization Algorithm}

Our optimization objective is stated below:

\begin{equation}
\Q^* = \argmin_{\Q \in \mathcal{Q}} L(\W, \Q).
\end{equation}

To solve this optimization problem, we use \emph{projected gradient descent}, which is stated in Algorithm \ref{algo:matmech}.

%\begin{enumerate}
%\item Initialize $\Q$ (e.g., using Hadamard strategy matrix)
%\item for $t = 1, \dots, T$
%\item $ \Q \leftarrow \Pi_{\mathcal{Q}} (\Q - \eta_t \nabla_{\Q} L(\W, \Q)) $
%\item return $\Q$
%\end{enumerate}
\begin{algorithm}[H]                   % enter the algorithm environment
\caption{}\label{algo:matmech}         % give the algorithm a caption
%\label{alg1}                           % and a label for \ref{} commands later in the document
\begin{algorithmic}                 % enter the algorithmic environment
      \STATE Initialize $\Q$ (e.g., using Hadamard strategy matrix)
         \FOR   {$t = 1, \dots, T$}
       \STATE  $ \Q \leftarrow \Pi_{\mathcal{Q}} (\Q - \eta_t \nabla_{\Q} L(\W, \Q)) .$
          \ENDFOR         
       \STATE Return  $\Q$
\end{algorithmic}
\end{algorithm}
The main technical challenge here is projecting onto the constraint set $\mathcal{Q}$.  It's straightforward to show that $\mathcal{Q}$ is the intersection of two convex sets (see proposition \ref{prop1}).

The alternating projection algorithm gives a method for projecting onto the intersection of these two sets, by repeatedly projecting onto each constraint in a sequential manner.  All we have to do is specify how to project onto each set individually.  It is well-known how to project onto the probability simplex \cite{wang2013projection}, but we will have to give our own algorithm for projecting onto the privacy constraint.  We have to solve the following problem:

\begin{equation*}
\begin{aligned}
& \underset{\hat{\q}}{\text{minimize}}
& & \norm{\q - \hat{\q}}_2^2 \\
& \text{subject to}
& & \hat{\q}_o \leq \exp{(\epsilon)} \hat{\q}_{o'} & \forall o, o',
\end{aligned}
\end{equation*}
where $\q$ is some vector, which we can interpret as one row of the strategy matrix.  We can translate this into a minimization problem over a single variable, $l$ which is (a lower bound on) the minimum value in $\hat{\q}$.  $\exp{(\epsilon)} l$ is (an upper bound on) the maximum value in $\hat{\q}$.  For a given value of $l$, $\hat{\q}$ can be derived from $\q$ by truncating each entry to the lie in the interval $[l, \exp{(\epsilon)} l]$.  We know the optimal value of $l$ lies within the range $[\min(\q), \max(\q)/\exp{(\epsilon)}]$ and we can find it by performing a binary search on the derivative function to find where it is zero.

Note that while the constraint set is convex, the objective function is not.  It is easy to verify this computationally by generating random strategy matrices and checking the definition of convexity directly.  Thus, we do not have convergence guarantees to a global minimum.  However, we can show that the error we get from our mechanism is never worse than the error of the mechanims in Table \ref{table:stdmech}.  This is because we can initialize the optimization with the best strategy matrix in Table \ref{table:stdmech}, and the returned solution will never be worse than that.


==> response.tex <==
%!TEX root = paper.tex

%{
%\setlength\parindent{0pt}
%\setlength{\parskip}{.5em}
%\newcounter{reviewcounter}
%\setcounter{reviewcounter}{0}
%\newcounter{commentcounter}[reviewcounter]
%\setcounter{commentcounter}{0}
%\renewcommand{\thecommentcounter}{\arabic{reviewcounter}.\alph{commentcounter}}

%\newenvironment{metareview}
%{
%	\begin{quote}
%
%	\color{black}
%}
%{\end{quote}}

\clearpage

\newcommand{\rc}[1]{{\it #1}}

\newenvironment{reviewcomment}
{
	\refstepcounter{commentcounter}
	R\thecommentcounter: \begin{quote} \color{black}
}
{\end{quote}}

\newenvironment{response}
{ \color{blue}
{\bf Author response:}
}
{}

\setcounter{page}{1}
%\newenvironment{reviewcomment}
%{
%	Author response: \color{blue}
%}
%{}

\vspace{3em}
\centerline{\Large\bf Note to the reviewers}
\vspace{1em}

We thank the reviewers for their thoughtful reviews and for the opportunity to improve our paper through revision.  
%Directly below we provide an overview of our revisions and responses to each reviewers' comments. 
We have revised the paper, making appropriate modifications to address reviewer comments.  All changes are highlighted in pink.  
Directly below we provide detailed responses to each reviewers' comments.

%\gm{there is no overview. It would be good to highlight the biggest changes made to the paper.}

%	\gm{Say that changes to the body of the paper are highlighted in PINK}

\vspace{1em}

{\Large \bf \noindent Reviewer 1}

\begin{description}
\item[R1.D1] \rc{It deserves more space to discuss the relationship (more formally) between matrix mechanism in the centralized setting and the mechanism in this work. In Section 6.1, it is said that 'To adapt the Matrix Mechanism to the local model, we run it independently for all N single-user databases and aggregate the results, as described in [18]." Then the question is what modification you did on the matrix mechanism to make it better for the local setting? The way you solve the optimization problem? Or, the way how the strategy matrix is designed?}

\begin{response}
The reviewer brings up a good point, and we have greatly expanded the discussion of the Matrix Mechanism in \cref{sec:related}, discussing in greater detail the similarities and differences between the Workload Factorization Mechanism proposed in this work and the Matrix Mechanism.

In Section 6.1 we compare our mechanism against a distributed version of the Matrix Mechanism, studied in \cite{edmonds2019power}.   This mechanism is a \emph{direct} application of the traditional Matrix Mechanism to LDP, without any modification to the optimization problem, strategy, or noise distribution in any way.  
%While typically thought of as a central DP mechanism, it was proposed as a mechanism for LDP in \cite{edmonds2019power} and studied in that context.  
We did not invent this approach, but simply treat it as a baseline to compare against, and we have made appropriate changes to Section 6.1 to clarify this.

The idea to translate central DP mechanisms to LDP was proposed in \cite{bassily2018linear}, where a LDP version of the Gaussian mechanism was studied (see Section 3.1 for the main idea).  The same translation was used for the Matrix Mechanism in \cite{edmonds2019power} and could in principle be used to translate \emph{any} central DP mechanism to LDP (for linear queries).  We have rewritten our discussion of these mechanisms in \cref{sec:related} to make this idea more clear.

%We have reworded the sentence to make it clear that this baseline approach is not our idea, but a previosly proposed mechanism.

%We do not fully understand the question, but will do our best to clarify the relationship between our mechanism and the Matrix Mechanism, both in this response and in the revised paper.  In Section 6.1 the mechanism we are calling the Matrix Mechanism is fully described (and thoroughly analyzed) in \cite{edmonds2019power}.  The mechanism they propose is a direct application of the (Gaussian) Matrix Mechanism to LDP, without any modification to the optimization problem or strategy in any way.  Unfortunately, they also call their mechanism the Factorization Mechanism.  To avoid a name conflict, we refer to it as the Matrix Mechanism, but we understand that is also a confusing name for two reasons: (1) The Matrix Mechanism is traditionally thought of as a central DP mechanism and (2) because our mechanism is inspired by and similar to the Matrix Mechanism at a high level, so the differences may not be obvious. 

%We hope the expanded discussion of the Matrix Mechanism we added to the related work will clear up these confusions for future readers.  
%\ry{perhaps a simpler solution is to just rename $L_2$ Matrix Mechanism to Gaussian Factorization Mechanism}
\end{response}

\item[R1.D2] \rc{It is interesting to discuss whether the proposed mechanism can cover the LDP algorithm HIO in:
Wang et al., Answering Multi-Dimensional Analytical Queries under Local Differential Privacy, SIGMOD 2019
to support multi-dim range queries (which is more general than Hierarchical [14]).}

\begin{response}
Yes, the HIO mechanism can indeed be represented as a strategy matrix within our framework.  The translation is largely similar to how we translate the simpler Hierarchical mechanism \cite{cormode2019answering}.  Please see below the response to R1.D3 for a description of the encoding.
\end{response}

\item[R1.D3] \rc{At first, I was wondering whether the framework can cover the sampling trick which is essential in LDP algorithms (i.e., "Use sampling" in [14] and "HI v.s. HIO" in [Wang et al., SIGMOD 2019]). It seems to me that the answer is yes, as we can treat random sampling-mapping-perturbation (in Hierarchy [14] or HIO [Wang et al., SIGMOD 2019]) as a whole distribution. But now the question is: how to choose the size of the strategy matrix (i.e., the output range m)? The optimal value seems to depend on the workload itself - is there any principle on how to set it?}

\begin{response}
The reviewers intuition is correct that our framework can support the sampling trick common in LDP mechanisms.  For this to work, the sampled item (e.g., level in the hierarchy) must be treated as part of the output of the mechanism.  The strategy matrix $\Q$ encodes the conditional distribution of \emph{all} the outputs of the mechanism (given the user type), including the sampled item together with the output produced by the frequency oracle. 

Below we show how this encoding is done for the (binary) Hierarchical mechanism (i.e., the 1D version of the HIO mechanism).  Let's denote the strategy matrix for the frequency oracle $\bar{\Q}^{n}$ when it is defined over a domain of size $n$.  The strategy matrix for the Hierarchical mechanism can then be expressed in terms of the frequency oracle in the following manner. 
$$ Q_{o,u} = \frac{1}{h} \bar{Q}_{k,\floor{\frac{u}{2^{h-l}}}}^{2^l} $$
Above, $o = (l,k)$, where $l \in \set{1, \dots, h}$ is the sampled level in the hierarchy and $k$ is in the output domain of the frequency oracle. 

The equation above looks complicated at first glance, but the structure is more apparent when viewed in matrix form: %, $\Q$ has the following structure:
$$
\Q = \frac{1}{h}
\left[
\begin{array}{c c c}
\bar{\Q}^{2} &\otimes& \mathbf{1}_{\frac{n}{2}} \\
\bar{\Q}^{4} &\otimes& \mathbf{1}_{\frac{n}{4}} \\
& \vdots & \\
\bar{\Q}^{\frac{n}{2}} &\otimes& \mathbf{1}_2 \\
\bar{\Q}^{n} &\otimes& \mathbf{1}_1 \\
\end{array}
\right] 
\begin{array}{l}
\text{level } 1 \\ \text{level } 2 \\ \textcolor{white}{\vdots} \\ \text{level } h-1 \\ \text{level } h
\end{array}
$$

Above, $\otimes$ is the Kronecker product and $\mathbf{1}_{a}$ is a $ 1 \times a$ vector of ones.  The vector of ones in the equation serves to discretize the domain by merging buckets, allowing the frequency oracle to run over smaller domains.  

We have expanded the background section, giving more examples of how existing mechanisms can be encoded as a strategy matrix.  Additionally, we now state explicitly that any mechanism can be encoded as a strategy matrix, as long as $\U$ and $\O$ are finite.  The main challenge to encoding a strategy matrix is calculating $\Pr[\M(u) = o]$ for each $(o,u)$ (the entries of $\Q$).  Please see the response to R1.D4 for additional details about the changes made.  

%\gm{It is not clear what we changed in the paper in response to the above. If there is no room for the above discussion to go in the paper, may we should add a note to the full version.}

%\gm{Why don't we compare against that technique in the experiments?} 
%RM: HIO is equivalent Hierarchical for 1D range queries, and we dont use multi-dim range queries in experiments

Regarding the size of the strategy matrix, we agree with the reviewer that this is an important question not adequetely addressed in the previous version of the paper, and we have taken steps to address it in the revised version.  Specifically, we added \cref{fig:initialization} and \cref{sec:initialization} to the experiments to study the impact of $m$ on the quality of the optimized strategy.  We found that our optimization algorithm is quite robust to the choice of $m$, and produces (almost) equally good strategies across a wide variety of $m$ in the range $[2n, 16n]$.  In other experiments, we used a default value of $m = 4n$, as we found that worked well across experimental settings and struck a good balance between computational time and solution quality.  In real-world applications, we recommend doing a hyper-parameter search to find the best value of $m$ to get the most utility out of our mechanism.  
%We treat this value as a hyper-parameter that can be tuned on a case-by-case basis.  We didn't search through this hyper-parameter space in experiments (although doing so would have improved the results), and instead opted for a default value of $m=4n$, which we found worked reasonably well across all experimental settings.  To understand the impact of this hyper-parameter in greater detail, we added an additional figure and discussion to the experimental section, showing that our optimization algorithm is pretty robust and produces (almost) equally good strategies across a wide variety of hyper-parameter settings.


\end{response}

\item[R1.D4] \rc{Better to give more non-trivial examples (besides Random Response) about why previous mechanisms are special cases of the proposed mechanism (e.g., Hierarchy [14] or HIO [Wang et al., SIGMOD 2019], or Hadamard [2]). I understand it needs space - so I suggest Section 5 can be shortened, where the results are not very surprising and are not the main contribution of this work.}

\begin{response}
We expanded the background section, adding \cref{table:stdmech}, which shows how some existing mechanisms can be expressed as a strategy matrix within our framework.  While this table does not cover every mechanism that fits within our framework, it covers several non-trivial ones (including Hadamard) and provides useful insights into what existing strategies look like.  We chose to omit the Hierarchical, HIO, or Fourier mechanisms from this table, as including them would require too much new notation, and in turn negatively impact the readability.  Instead, we have open-sourced our code base for the interested reader, which includes functions to encode these mechanisms as strategy matrices.

%\gm{as above, it would be nice to say here that we added it to the full version.}
\end{response}

\item[R1.D5] \rc{How large is the domain that can be handled by the optimization algorithm? For example, for multi-dim range queries (with potentially large n = (attribute size)$^d$ and m), can we model and solve it using the proposed approach? If not (which is fine), what are the largest n and m that can be handled? If we use a relatively smaller m than needed, whether the error would be much larger}

\begin{response}
We discuss scalability of our optimization algorithm in \cref{sec:exp:scalability}.  The largest domain we ran on was $n=4096$.  In principle, it could be possible to scale up further with more time and computational resources, however.

%The nice thing about the workload of all range queries is that it is highly structured.  Thus, even though the number of queries is $O(n^2)$, we can exploit the structure to efficiently compute its Gram matrix $\W^T \W$, which is all that is needed for optimization.  This Gram matrix is $ n \times n $ and is substantially smaller than $\W$ itself.   
%
%In general, the number of queries in the workload is much less important than the size of the domain, because the objective function only depends on $\W$ through its Gram matrix $\W^T \W$, which only needs to be computed once prior to optimization.  Since the Gram matrix is $n \times n$, it is much smaller than $\W$ for very large workloads like all range queries.  Furthermore, for highly structured workloads, including all range queries, we can avoid materialzing $\W$ all together, and just compute $\W^T \W$ directly instead.  

%\ry{may be going on a tangent here... is this necessary?} \gm{keep it}
While it may be difficult to run our mechanism directly for domains much larger than this, we believe our mechanism may still be useful as a sub-routine for more scalable mechanisms.  For example, we could bypass the need to solve an intractable optimization problem for the special case of multi-dimensional range queries by dividing the privacy budget and invoking sequential composition.  There, each user runs $d$ small mechanisms for 1D range queries, rather than one big mechanism for $d$-dimensional range queries.  

This sequential composition is equivalent to using the strategy matrix $\Q = \Q_1 \otimes \dots \otimes \Q_d$, where $\Q_i$ is the strategy matrix for the $i^{th}$ mechanism and $\otimes$ is the Kronecker product \cite{mckenna2018optimizing}.  To estimate the workload query answers we could similarly use $ \V = \V_1 \otimes \dots \otimes \V_d$.

%\ry{I believe (although can't be sure) that this is equivalent to what HIO does in [Wang et al., SIGMOD 2019].  Although it is not described in that way, it is much more notationally clunky}

\end{response}
\end{description}

{\Large \bf \noindent Reviewer 2}

\begin{description}

\item[R2.D1] \rc{It will be natural to assume the rank of a $p \times n$ workload matrix is $\min(p,n)$.  Does this assumption make the discussion simpler?}

\begin{response}
This is a good point, as many common workloads will naturally have rank $\min(p,n)$.  In fact, four workloads we used in experiments have rank $n$ (Histogram, Prefix, All Range, and All Marginals).  

When the rank of $\W$ is $n$, the rank of $\Q$ must also be $n$, in which case we can replace $(\Q^T \D^{-1} \Q)^\dag$ with $(\Q^T \D^{-1} \Q)^{-1}$.  This assumption does make some of the proofs go through easier, although it does not change or simplify the main discussion much.  

Because this assumption only affects the proofs, and not the main text, we believe the loss of generality is not worth the simpler proofs.  A very nice feature of our mechanism is that the workload can be completely arbitrary, as we make no assumptions about its structure or contents.  This gives the analyst great flexibility when constructing the workload.   We added a discussion of this point after \cref{ex:prefix}.

Computationally, evaluating the objective function (and hence optimizing the strategy) is easier when the rank is $n$, because it is generally more efficient to calculate the inverse instead than the pseudo inverse.  
%\ry{Do we need to discuss computational considerations when rank is $n$?} \gm{I think it is okay as is}

%While the other two workloads do not have rank $\min(p,n)$, there should exist a rank $\min(p,n)$ ``surrogate'' workload that is equivalent to the original for the purposes of optimization --- i.e., they have the same Gram matrix and hence define the same objective function.
\end{response}

\item[R2.D2] \rc{Does the simplification of $\W$ affect the problem?  For example, is the matrix in Example 2.4 essentially the same with a unit matrix?}

\begin{response}
It is true that any strategy that supports (i.e., provides unbiased answers to) the workload in Example 2.4 will also support the unit/Identity matrix, since they both have rank $n$.  However, these workloads do define different objective functions, and different factorizations will be needed for each.  This is why it is so important for the analyst to specify \emph{all} queries they care about, not just the ones needed to construct an appropriate view of the data from which other queries can be estimated.  In \cref{sec:experiments}, we note that all mechanisms can run on all workloads with minor modifications, but observe that the best-performing mechanisms are the ones that are tailored to the workload. 

%\ry{Where can we add sentence to emphasize this point?  It is already mentioned in a couple places.}
\end{response}

\end{description}

{\Large \bf \noindent Reviewer 3}

\begin{description}

\item[R3.D1] \rc{The main weakness of the current paper lies in the evaluation section.}

\item[R3.D1.1] \rc{ There are no experiment results on real dataset. In addition to directly translating calculations of the theoretical results into figures (e.g. Corollary 5.4 to Figure 1,2), it would be better to include experiments on real datasets and show the benefit of the approach in terms of utility compared to baseline approaches.}

\begin{response}
We agree with the reviewer that this is an important question to understand and deserves further investigation and discussion.  

We believe it makes sense to use the sample complexity corresponding to the worst-case variance as the primary evaluation metric in \cref{fig:workload-eps} and \cref{fig:workload-domain}, as it is our stated objective to optimize this (\cref{prob:optimization}) and it is a tight universal bound that holds for \emph{all possible} data sets.  Furthermore, in real-world applications of the mechanism, it is important to check the expected error before running the mechanism, so an appropriate privacy budget can be chosen.  Since the true data is unavailable for this purpose (as it is a private quantity), the next best alternative is to use the expected utility on the worst-case dataset (i.e., worst-case variance). 

We have therefore kept \cref{fig:workload-eps} and \cref{fig:workload-domain} as is, and added \cref{sec:exp:dataset} and \cref{fig:dataset} to evaluate the performance of our mechanism on real-world benchmark datasets.  
%That being said, we agree that it is also important to evaluate the performance on real-world datasets as well.  We have therefore added \cref{sec:exp:dataset} and \cref{fig:dataset} to understand the impact of the dataset on the results.  
Our main finding is that the dataset does not impact the results much at all, and the performance of all mechanisms are quite consistent across all the datasets we tested.  Furthermore, we found that the worst-case variance/sample complexity is an excellent proxy for the real-world variance/sample-complexity.  Intuitively, this behavior is expected, as the privacy guarantee requires the mechanism to perform similarly for all user types.  This intuition was used to prove the related result that the worst-case variance is tightly bounded above and below by the average-case variance (\cref{thm:avg_worst}).  

\end{response}


\item[R3.D1.2] \rc{For the evaluation metric, the experiments compare the proposed algorithm with baselines mainly under the sample complexity metric. How would the comparisons look like under workload specific utility metrics, especially when comparing the proposed algorithm with algorithms optimized specifically for a particular utility measure (if there is any).}

\begin{response}
Existing work on this task have mainly considered the $L_1$ error \cite{acharya2018hadamard,ye2018optimal,cormode2018marginal}, $L_2$ squared error \cite{erlingsson2014rappor,bassily2018linear,cormode2019answering,acharya2018hadamard,edmonds2019power,wang2017locally}, and $L_{\infty}$ error \cite{edmonds2019power} as the primary evaluation metrics.  In this work, we chose to work with the $L_2$ squared error (total variance for unbiased mechanisms), for its nice analytical and smoothness properties.  Because our stated objective is to design a mechanism with low expected $L_2$ squared error, we believe it makes sense to compare mechanisms on that metric as we did.  
However, since it is difficult to interpret these error values directly, we opted to report the sample complexity instead, or the number of samples required to obtain a sufficiently low expected $L_2$ squared error.  The number of samples is a more intuitive unit to quantify and compare mechanism performance.      

It is an interesting avenue for future research to see whether improvements in $L_2$ squared error translate into improvements in other error metrics as well, although we consider that beyond the scope of this work.
\end{response}

\item[R3.D1.3] \rc{Finally, it would be good to show how the output $\Q$ looks like for a particular workload (e.g. Histogram), how is the consistency of $\Q$ from different runs, and how different $\Q$ is compared to a known LDP mechanism.}

\begin{response}
This is an interesting empirical question, and something we have looked into.  
When visualizing the strategies produced by our optimization algorithm, we find it difficult to discern a clear interpretable structure, making it challenging to extract useful insights from them.  Below we show a strategy obtained by optimizing the Histogram workload with $n=8$ and $\epsilon=1.0$.

\begin{figure}[h]
\centering
\includegraphics[width=0.3\textwidth]{fig/histogram-viz}
\end{figure}

%In many cases, it is difficult to interpret the strategy produced by our optimization algorithm, and it usually looks quite different than the strategies of the other mechanisms we compared against.  In some limited cases structure does emerge, however. For example, the strategy produced by our mechanism seems to converge towards randomized response for large $\epsilon$.  

Regarding the consistency between runs, we agree with the reviewer that this an in important question not addressed in the previous version of the paper.  We have updated the experiments, adding \cref{fig:initialization} and \cref{sec:initialization} to include a result on the consistency between runs.  We show that our optimization algorithm is quite robust to the random initialization, as the quality of the strategies produced from different random initialization do not change significantly.  That being said, with enough time and resources, randomly restarting the optimization to find better strategies cannot hurt.  
\end{response}

\item[R3.D2] \rc{Some descriptions of the technical content can be made more clear.}

\item[R3.D2.1] \rc{For example, the relation between the sequence of $o_i = \M_{\Q}(u_i)$, $y_o, \M_{\Q}(\x)=\y$ at the end of Sec.2 and $\M_{\Q}(\x) = \Q \x$ in Sec. 3 is a bit confusing. Because of this, the proof of Thm 3.4 is also not clear, e.g. why $\z_u$ is a multinomial random variable with trials number $x_u$ and probability $\q_u$? Also, For Proof of Theorem 3.4, please give more information about the equation of $Cov[\z_u]$, such as 1) how this equation is derived; 2) what’s the meaning of bold $\mathbf{p}$.}

\begin{response}
We added supporting text at the end of Section 2 to explain some of the notational choices more clearly, and we also updated the proof of Theorem 3.4 to address concerns there.
\end{response}

\item[R3.D2.2] \rc{The introduction of the reconstruction matrix $\V$ is not well-explained. Please provide some intuition for introducing this matrix, why should it be a linear factor to $\Q$ without any constraints, can it be replaced by a nonlinear transform on $\Q$ and lead to better performance?}

\begin{response}
We reorganized the discussion immediately following \cref{def:factorization} to better explain the purpose of $\V$.   As we hinted at at the end of Section 2, the response vector produced by $\M_{\Q}$ is not that useful by itself, and it must be post-processed to estimate more useful quantities.  $\V$ serves that purpose, as it is used to estimate the workload-query answers.  The only constraint on $\V$ is that $\W = \V \Q$, which is needed to ensure the estimates produced by the mechanism are unbiased.
%\ry{do we need to address the nonlinear transform question?  Might convolute the text, but can discuss it more in the response maybe}  \gm{I think it would be enough to describe it briefly in the response.}

If we wanted to replace $\V$ with a non-linear transformation $f$, we would need $ \W \x = f(\Q \x) $ for all $\x$ to achieve unbiasedness.  It's not clear whether such a transformation exists, other than the linear transform we use.  Furthermore, the simplicity of the linear transform allowed us to derive a closed form expression for the optimal $\V$, as well as a compact expression for the objective function in terms of linear algebra primitives.

\end{response}

\item[R3.D2.3] \rc{It would be better to give explanation or definition for the parameter $\lambda$ when it first appeared in Proposition 4.2.}

\begin{response}
We added a sentence explaining what $\lambda_u$ represents and where it comes from after \cref{prop:projection}.

%\ry{is it enough? can we reference [44]?}
%The vector $\boldsymbol{\lambda} = [\lambda_u]_{u \in \U}$ is a Lagrange multiplier for the equality constraint $ \Q^T \mathbf{1} = \mathbf{1}$ in \cref{prob:projection}.  
\end{response}

\item[R3.D2.4] \rc{For Problem 3.12, does the variable $\z$ mean the same thing as it does in Proof of Theorem 3.4? If yes, in Problem 3.12, it seems like the variable $\z$ is a minimum allowable value on $\q_u$, while in Proof of Theorem 3.4, that $\z$ is a multinormal variable instantiated with $\x$ and $\q$.}

\begin{response}
The reviewer is correct to point out that these are two different usages of the same symbol $\z$.  We changed $\z_u$ to $\mathbf{s}_u$ in the proof of \cref{thm:variance}, and reviewed the rest of the document for symbol reuse.  
\end{response}
\end{description}



==> result.tex <==
\section{Results}
In this section we experimentally compare our mechanism against the Hadamard mechanism and Randomized Response mechanism described in table \ref{table:stdmech}.  We omit from comparison RAPPOR and Subset Selection due to the exponential size of their strategy matrix.

We evaluate these mechanims using expected error on three commonly studied workloads (Identity, Prefix, and Width 20 Range) for a fixed domain size of $n=128$.  Identity is the simple $n \times n$ identity matrix, Prefix is the $n \times n$ lower triangular matrix of ones, and Width 20 Range is the $n-20 \times n$ matrix where row $ \w_i $ is $1$ at indices $i$ through $i+20$ and $0$ otherwise.  Because the expected error depends on the true data vector $\x$, we report \emph{worst-case} error as well as error on a real-world benchmark dataset \cite{hay2016principled}.  Additionally, we normalize the error and report Root-Mean-Squared-Error:

$$ {\rm RMSE} = \sqrt{\frac{{\rm Error}(\W,\Q,\x)}{m}}.$$ 

\begin{figure}[h!]%
\begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{newplot/Prefix_Total_Patent_128.png} % first figure itself
       %\caption{$ \sqrt{\frac{\text{Total variance}}{\text{Number of queries}}}$ vs epsilon for Prefix query }
    \end{minipage}\hfill
    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{newplot/Prefix_worst_Patent_128.png} % second figure itself
        %\caption{worst case error vs epsilon for Prefix query}
    \end{minipage}
    \caption{Expected real-word error (left) and worst-case error (right) on the Prefix workload.}
    \label{Prefix}
\end{figure}



\begin{figure}[h!]%
\begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{newplot/Identity_Total_Patent_128.png} % first figure itself
       %\caption{$ \sqrt{\frac{\text{Total variance}}{\text{Number of queries}}}$ vs epsilon for Identity workload }
    \end{minipage}\hfill
    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{newplot/Identity_worst_Patent_128.png} % second figure itself
        %\caption{worst case error vs epsilon for Identity workload }
    \end{minipage}
    \caption{Expected real-word error (left) and worst-case error (right) on the Identity workload.}
    \label{Identity}
\end{figure}

\begin{figure}[h!]%
\begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{newplot/Range_Total_Patent_128.png} % first figure itself
       %\caption{$ \sqrt{\frac{\text{Total variance}}{\text{Number of queries}}}$ vs epsilon for Identity workload }
    \end{minipage}\hfill
    \begin{minipage}{0.23\textwidth}
        \centering
        \includegraphics[width=0.95\textwidth]{newplot/Range_worst_Patent_128.png} % second figure itself
        %\caption{worst case error vs epsilon for Identity workload }
    \end{minipage}
    \caption{Expected real-word error (left) and worst-case error (right) on the Width 20 Range workload.}
    \label{Range}
\end{figure}

We consider seven different values of $\epsilon= [ 0.1,0.4,0.7,1,1.5,2,5] $ and plot the results in Figures \ref{Prefix}, \ref{Identity}  and \ref{Range}. For both the Prefix workload and Width 20 Range workload, our method consistently outperforms the competitors at all privacy levels by around a factor of 1.8.  For the Identity workload, our method is competitive with and slightly better than the Hadamard mechanism in the high privacy regime (low $\epsilon$), and better than both mechanisms in the low privacy regime.  

The amount of time it requires to solve the optimization problem using our algorithm varies by workload and $\epsilon$ -- it can be as low as a few seconds and as high as a few minutes.


==> running.tex <==
\section{Running the Mechanism}

In this section, we bring it all together and state the full mechanism, including how to use it to estimate the data vector (not just the workload answers).  The full mechanism is stated in \cref{alg:ldpmm}.  Each iteration of the for loop is to be executed independently on each users device, before sending the randomized responses $o_i$ to the server. 


\begin{algorithm}[h]                   % enter the algorithm environment
\caption{}\label{alg:ldpmm}         % give the algorithm a caption
%\label{alg1}                           % and a label for \ref{} commands later in the document
\begin{algorithmic}                 % enter the algorithmic environment
\STATE optimize $\Q$ using \cref{alg:matmech}
\STATE calculate $\V$ using \cref{thm:optv}
\STATE $\y = \mathbf{0}$
\FOR {$i = 1, \dots N$}
\STATE $ o_i \sim \q_{u_i} $
\STATE $y_{o_i}$ += 1
\ENDFOR
\STATE \textbf{return} $\V \y$
\end{algorithmic}
\end{algorithm}

\subsection{Extension: Non-negativity and Consistency} \label{sec:wnnls}

We have now completely described our mechanism.  Now, we describe a simple extension that can improve the utility in practice.  While our basic mechanism offers unbiased answers to the workload queries, this can come at the cost of certain anomalies.  For example, the estimated answer to a workload query might be negative, even though the true answer could never be negative.  This motivates us to consider an extension where we try to account for the structural constraints we know about data vector.  Specifically, we propose the following non-negative least squares problem to find a non-negative (feasible) $\hat{\x}$ such that $ \W \hat{\x}$ is as close as possible to our unbiased estimate $\V \y$.  Formally, the problem at hand is:

$$\hat{\x} = \argmin_{\x \geq 0} \norm{\W \x - \V \y}_2^2$$

Once $\hat{\x}$ is obtained, the workload answers can be estimated by computing $\W \hat{\x}$.  While this estimate is not necessarily unbiased, it often has substantially lower variance than $\V \y$ and can be a worthwhile tradeoff, particularly in the high-privacy/low-data regime where non-negativity is a bigger issue.
A similar problem was studied theoretically by Nikolov et al. \cite{nikolov2013geometry} and empirically by Li et al. \cite{li2015matrix} in the central model of differential privacy, where it has been shown to offer significant utility improvements.  There are various python implementations to solve the above problem efficiently \cite{scipy,zhang2018ektelo,mckenna19graphical}.  We simply use the limited memory BFGS algorithm from scipy to solve it \cite{scipy}.  

